Restyling Data: Application to Unsupervised Domain Adaptation

Machine learning is driven by data, yet while their availability is constantly increasing, training data require laborious, time consuming and error-prone labelling or ground truth acquisition, which in some cases is very difficult or even impossible. Recent works have resorted to synthetic data generation, but the inferior performance of models trained on synthetic data when applied to the real world, introduced the challenge of unsupervised domain adaptation. In this work we investigate an unsupervised domain adaptation technique that descends from another perspective, in order to avoid the complexity of adversarial training and cycle consistencies. We exploit the recent advances in photorealistic style transfer and take a fully data driven approach. While this concept is already implicitly formulated within the intricate objectives of domain adaptation GANs, we take an explicit approach and apply it directly as data pre-processing. The resulting technique is scalable, efficient and easy to implement, offers competitive performance to the complex state-of-the-art alternatives and can open up new pathways for domain adaptation.

==> figures/gta2cityscapes.tex <==


%Old
%From top to bottom: trained on GTA only, %\srcTarget{GTA}{RS-tgt}{tgt}, %\srcTarget{GTA}{PH-tgt}(tgt). Best viewed in %color}

%\iffalse
%\begin{figure}[h!]
%        \begin{adjustbox}{minipage=\linewidth,scale=0.45}
%        \begin{subfigure}[b]{0.0001\textwidth}
%                \includegraphics[width=\linewidth]{figures/img/source_only_city.png}
%                \caption{Source only}
%                \label{Source only}
%        \end{subfigure}%
%        \begin{subfigure}[b]{0.0001\textwidth}
%                \includegraphics[width=\linewidth]{figures/img/random_city.png}
%                \caption{Random styles}
%                \label{Random styles}
%        \end{subfigure}%
%        \begin{subfigure}[b]{0.0001\textwidth}
%                \includegraphics[width=\linewidth]{figures/img/ph_cityscapes.png}
%                \caption{With perceptual hashing matching}
%                \label{With perceptual hashing matching}
%        \end{subfigure}%
%        \begin{subfigure}[b]{0.0001\textwidth}
%                \includegraphics[width=\linewidth]{figures/img/gt_city.png}
%                \caption{Ground truth}
%                \label{Ground truth}
%        \end{subfigure}%
%         \begin{subfigure}[b]{0.0001\textwidth}
%                \includegraphics[width=\linewidth]{figures/img/original_city.png}
%                \caption{Real image}
%                \label{real}
%        \end{subfigure}%
%        \end{adjustbox}
%        \caption{Predictions maps for $GTA \rightarrow Cityscapes$}\label{fig:animals}
%\end{figure}

==> figures/gta2mapillary_predictions.tex <==

%\begin{figure*}[h!]
%       \begin{subfigure}[t]{0.2\textwidth}
%            \includegraphics[scale=0.14]{figures/img/baseline_zRmo-YLdunzlwFVQv1EOyg111.png}
%            \caption{Source only}
%        \end{subfigure}
%        \begin{subfigure}[t]{0.2\textwidth}
%            \includegraphics[scale=0.13]{figures/img/random_zRmo-YLdunzlwFVQv1EOyg111.png}    
%            \caption{Random styles}
%        \end{subfigure}%
%        \begin{subfigure}[t]{0.2\textwidth}
%            \includegraphics[scale=0.13]{figures/img/hash_zRmo-YLdunzlwFVQv1EOyg111.png}
%            \caption{With perceptual hashing matching}
%        \end{subfigure}%
%        \begin{subfigure}[t]{0.2\textwidth}
%            \includegraphics[scale=0.13]{figures/img/zRmo-YLdunzlwFVQv1EOyg_gt.png}
%            \caption{Ground truth}
%        \end{subfigure}%
%        \begin{subfigure}[t]{0.2\textwidth}
%            \includegraphics[scale=0.13]{figures/img/real_zRmo-YLdunzlwFVQv1EOyg.png}
%            \caption{Real Mapillary image}
%        \end{subfigure}%
%\caption{Predictions maps for $GTA \rightarrow Mapillary(target)$}\label{fig:GTA2Mapillary}
%\end{figure*}

==> tables/resultsMNIST_USPS_SVHN.tex <==
\begin{table}[!ht]
    \caption{Experimental results on unsupervised domain adaptation for the digit classification task using the MNIST and SVHN datasets. Accuracy gains with respect to each method's baseline are reported in parenthesis.}
    \label{table:digits}
    \centering
    %\resizebox{\columnwidth}{!}{
    \small{
        \begin{tabular}{ l | c } 
            \hline
            $Method$ & $SVHN\rightarrow MNIST$ \\ 
            \hline \hline
            %$Source only  & 75.2 & 57.1 & 60.1 \\
        	%$Revgrad$ \cite{revgrad}  & - & - & 73.91 \\
        	$DANN$ \cite{ganin2015unsupervised, GaninJournal}
              & 73.85 (+18.95) \\
            \hline
            
            DRCN \cite{Ghifary2016DeepRN}
             & 81.97 (+19.64) \\ 
            \hline
            
            $ADDA$ \cite{AddaTzeng}
             & 76.0 (+15.9)  \\ 
            \hline
            
            $CyCADA$ \cite{CyCADA}
            & 90.4 (\textbf{+23.3})  \\ 
            \hline
            Murez et al. \cite{im2im2} & \textbf{92.1} (+12.1)\\ 
            \hline

             Ours (RS) & 74.25 (+5.22)   \\
            \hline
        \end{tabular}
    }
\end{table}
